Data-Driven Collective Variables for Enhanced Sampling

Designing an appropriate set of collective variables is crucial to the success of several enhanced sampling methods. Here we focus on how to obtain such variables from information limited to the metastable states. We characterize these states by a large set of descriptors and employ neural networks to compress this information in a lower-dimensional space, using Fisher's linear discriminant as an objective function to maximize the discriminative power of the network. We test this method on alanine dipeptide, using the non-linearly separable dataset composed by atomic distances. We then study an intermolecular aldol reaction characterized by a concerted mechanism. The resulting variables are able to promote sampling by drawing non-linear paths in the physical space connecting the fluctuations between metastable basins. Lastly, we interpret the behavior of the neural network by studying its relation to the physical variables. Through the identification of its most relevant features, we are able to gain chemical insight into the process.

==> arxiv/abstract_v1.tex <==
\begin{abstract}
Designing an appropriate set of collective variables is crucial to the success of several enhanced sampling methods. Here we focus on how to obtain such variables from information limited to the metastable states. We characterize the states by a large set of descriptors and employ neural networks to compress this information on a lower-dimensional space, using Fisher's linear discriminant as objective function to maximize the discriminative power of the network. 
We benchmark this method on alanine dipeptide, using the non-linearly separable dataset composed by atomic distances. We then study an intermolecular aldol reaction characterized by a concerted mechanism. 
The resulting variables are able to promote sampling by drawing non-linear paths in the physical space connecting the fluctuations between metastable basins.
Lastly, we inspect the behavior of the neural network by studying its relation to physical variables. Through the identification of its most relevant features, we are able to gain chemical insight into the process.
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7 \columnwidth]{figures/graphical_abstract.png}
\end{figure}
% keywords can be removed
\keywords{Enhanced sampling $|$ Collective variables $|$ Deep learning} 
\end{abstract}

==> arxiv/paper_v1.tex <==
\section*{Introduction}
In the last decades, enhanced sampling methods have become one of the main tools of contemporary science. They have managed to extend the scope of atomistic simulations, thus allowing long time scale phenomena to be simulated. Starting from the pioneering work of Torrie and Valleau \cite{Torrie1977}, a large class of such methods relies on the introduction of collective variables (CVs) defined as functions of the atomic coordinates. Once these variables are identified, to accelerate sampling a bias potential is added to the interaction potential  \cite{Valsson2016}. 
In order to achieve this goal, the CVs are chosen so as to describe the hard-to-sample modes of the system. Not surprisingly, much effort has been devoted to the identification and improvement of useful CVs. Very recently, machine learning methods with different levels of complexity have been also used to this effect \cite{Ma2005,Ribeiro2018,Chen2018,Schoberl2019a,Rogal2019,Ravindra2019}. Here we describe a new method that is based on deep neural networks (NNs). However, before describing our approach we recall some recent findings that give a clue to what we plan to do.

The free energy landscape of physical systems can be described as made up of islands of metastability in a sea of improbable configurations. The metastable states are connected by narrow passageways that allow rare but crucial transitions from one state to another to take place. Very recently our group and others \cite{Mendels2018,Sultan2018} have developed a family of efficient CVs based only on the fluctuations that the system undergoes in the metastable basins. This defies the conventional wisdom that for a variable to be effective, it must contain explicit information about the whole reaction path or at least the transition state \cite{Ma2005,Peters2017}. 

As an example of this approach, we briefly recall how the method called harmonic linear discriminant analysis (HLDA) \cite{Mendels2018} works. One first identifies a small set of descriptors capable of discriminating between the states. The expectation value of the descriptors and their covariance matrices are computed from short unbiased runs in the two basins. With the knowledge of only these quantities, and by using a variant of the classification method that goes under the name of linear discriminant analysis (LDA) \cite{welling2005}, one obtains CVs that are linear combinations of the input descriptors.

This simple approach has proven to be highly effective in a number of examples \cite{Piccini2018,Mendels2018a,Rizzi2019} but presents two limitations. At first, its linearity makes it not very effective in describing complex processes.
%by construction the HLDA CV is a linear combination of the descriptors. In complex examples, a linear may struggle in capturing the complexity / somewhat simplistic picture
Secondly, it relies on the identification of a small set of uncorrelated descriptors. While this is a far less demanding task than finding CVs, it requires knowledge of the system and physical intuition. This intuition can be of great help in leading to an accelerated sampling, however, it sometimes reflects more our prejudice than the actual system behavior, possibly preventing the exploration of some of the relevant transition pathways. With the use of an appropriately designed neural network, we want to lift these two limitations and construct a minimal set of CVs in order to study rare events.

\section*{Method}
Once the purpose has been clarified, we describe our approach. We want to generalize the previous work of HLDA by employing a neural network and casting LDA as the objective function. This can be seen as a non-linear generalization of LDA, as proposed already in the context of computer science for classification purposes \cite{Dorfer2016}. Consider a set of $N$ data points $\mathbf{x}_1,...,\mathbf{x}_N$ (observations) of dimension $d$ (local descriptors) belonging to $C$ classes (metastable states). The covariance matrix over all these samples can be decomposed in two terms, the so-called between class and within class scatter matrices. The former takes into account the fluctuations inside the basins, and corresponds to the average of the class covariances $\mathbf{S}_i$:
\begin{equation}
    \mathbf{S}_w = \frac{1}{C} \sum_i ^C \mathbf{S}_i.
\end{equation}
On the other hand, $\mathbf{S}_b$ is defined as the covariance of the class means $\bm{\mu}_i$, and thus measures the fluctuations between classes:
\begin{equation}
    \mathbf{S}_b = \frac{1}{C} \sum_i ^C (\bm{\mu}_i -\bm{\mu})(\bm{\mu}_i -\bm{\mu})^T
\end{equation}
where $\bm{\mu}$ is the average of the $C$ class means.
Fisher's criterion seeks a linear projection $\mathbf{W}$ into a $C-1$ dimensional space, such that the samples show a high variance between classes and a low variance within. This is achieved by maximizing Fisher's ratio: 
\begin{equation}
    \argmax_\mathbf{W} \frac{\mathbf{W} \mathbf{S}_b \mathbf{W}^T}{\mathbf{W} \mathbf{S}_w \mathbf{W}^T}.
    \label{eq:fisher}
\end{equation}
%where $\mathbf{S}_b$ and $\mathbf{S}_w$ are the so-called between class and within class scatter matrices. %The latter is defined as the mean of the covariance matrices $\mathbf{S}_i$ in the different states:

%The between class scatter matrix is defined as sample covariance of the class means $\bm{\mu}_i$, with $\bm{\mu}$ being the average of class means:

%We note that another way to compute $\mathbf{S}_w$ is using the total scatter matrix $\mathbf{S}_t$, which corresponds to the covariance matrix over the entire population, as $\mathbf{S}_b = \mathbf{S}_t - \mathbf{S}_w$.
In order to find the combination $\mathbf{W}$ which maximizes eq. \ref{eq:fisher}, one has to solve the generalized eigenvalue problem:
\begin{equation}
    \mathbf{S}_b \mathbf{w} = \mathbf{v} \mathbf{S}_w \mathbf{w}
    \label{eq:eig-problem}
\end{equation}
where the eigenvectors $\mathbf{w}$ form the projection matrix $\mathbf{W}$ and the eigenvalues $\mathbf{v}$ quantify the separation in the corresponding directions.  

\begin{figure}[t]
  \centering
  \includegraphics[width=0.75
  \columnwidth]{figures/DeepLDA_labels.png}
  \caption{Scheme of the construction of the Deep-LDA CV. A set of physical descriptors are used as inputs of a feed-forward neural network. The objective is to maximize the eigenvalues of LDA on the topmost hidden representation. The corresponding eigenvectors are then used to project the last layer onto a set of CVs.}
  \label{fig:method}
\end{figure}

We now illustrate how LDA can be used to train a neural network. We feed a number of descriptors to the NN that reduces the dimensionality of the data through a succession of continuous non-linear transformations represented by $f_\theta(\mathbf{x})$ with parameters $\theta$ (see fig. \ref{fig:method}).
We then compute LDA on the topmost hidden space representation $\mathbf{h}=f_\theta(\mathbf{x})$, and use the eigenvalues in the objective function to optimize the parameters of the NN. In the typical case of a two-classes problem, this corresponds to maximizing the single relevant eigenvalue, while for multi-states problems one can either use the smallest of the $C-1$ eigenvalues or their sum \cite{Dorfer2016}. Therefore, one increases the discriminative power of the neural network, by learning at the same time linearly separable latent features. Lastly, the hidden features are projected along the eigenvectors to obtain a minimal set of CVs. This formulation allows handling a large number of inputs, which do not need to be linearly separable and can also be correlated. We refer to this method as Deep-LDA CV. 

%In order to optimize the NN with backpropagation, we need the gradients of the eigenvalues, but, in general, machine learning libraries do not provide them for generalized eigenvalue problems. One possible way to solve this is by explicitly computing the partial derivatives of the eigenvalues with respect to the topmost hidden representation $\mathbf{h}$ \cite{Dorfer2016}.
%Here we follow another strategy \cite{Chen2019}, exploiting the fact that the scatter matrices are symmetric. We apply a Cholesky decomposition to $\mathbf{S}_w = \mathbf{L}\ \mathbf{L}^T$ and with standard algebra we rewrite the generalized problem of eq. \ref{eq:eig-problem} as follows:

In practice, we transform the generalized eigenvalue problem into a standard one by making first a Cholesky decomposition of $\mathbf{S}_w = \mathbf{L}\ \mathbf{L}^T$ \cite{welling2005}. By simple manipulation, we rewrite eq. \ref{eq:eig-problem} as:
\begin{equation}
    \widetilde{\mathbf{S}}\ \widetilde{\mathbf{w}}_i = v_i\  \widetilde{\mathbf{w}}_i
\end{equation}
where $\widetilde{\mathbf{S}}=\mathbf{L}^{-1} \mathbf{S}_b (\mathbf{L}^T)^{-1}$ and $\widetilde{\mathbf{w}}_i=(\mathbf{L}^T)^{-1}\ \mathbf{w}_i$. This way, we have a symmetric eigenvalue problem which can be solved within the Pytorch library \cite{AdamPaszke;SamGross;etal2017}. This allows training Deep-LDA networks with backpropagation and mini-batch gradient descent, provided that the batch-size is large enough to be representative of the population.

To make the LDA cost function more suitable for neural network optimization and to stabilize smaller eigenvalues, we follow \cite{Dorfer2016} and regularize the within scatter matrix by adding a multiple of the identity matrix $\mathbf{S}_w+\lambda\mathbf{I}$. 
Since we want to use the output of the NN to enhance sampling rather than classifying, we prevent the projected states from becoming too narrow. To enforce this, we include a penalty term on the distance between the states along the CV $s$, defined in a smooth way by a Lorentzian function:
\begin{equation}
    \mathcal{L}_s = - \frac{1}{1+\left(\frac{1}{n_b\ n_{cv}}\sum_{b,i} s_i ^2 (\mathbf{x}_b) -1\right)^2}
    \label{eq:lorentzian}
\end{equation}
where the sum goes over the elements $b$ in the batch and the CV dimensions $i$. In addition, a standard L2 regularizing term is used (see \ref{sec:S-nn} for the details).
%Both $\alpha$ and $\lambda$ are hyper-parameters, even tough we found them to be connected and thus we choose them accordingly. 
%An intuitive picture of the interaction of the terms in the loss function during training is as follows....
%nd is able to represent more accurately the non-linear nature of complex processes by gently joining the fluctuations in different basins. %the non-linearity lets the CV follow the unbiased fluctuations across all the states, effectively drawing a path in the descriptors space. To better illustrate this, we shall refer to the example of realistic applications.

After training our CV, we use it in combination with enhanced sampling methods. This could be done with any CV-based methods, such as Metadynamics \cite{Laio2002} or Variational enhanced sampling \cite{Valsson2014,Bonati17641}. In this work, we choose to employ a recently developed variant of Metadynamics, called on-the-fly probability enhanced sampling (OPES) \cite{Invernizzi2019}, which is based on a Gaussian modeling of the probability distribution estimate. The main benefits of OPES are the small number of free parameters, the ability to limit the exploration in the CV space to the desired process, and a faster convergence than Metadynamics. In OPES one establishes the following relation between the unbiased probability $P_n(\mathbf{s})$ and the bias potential $V_n(\mathbf{s})$:
\begin{equation}
    V_n(\mathbf{s}) = \left(1-\frac{1}{\gamma}\right)\frac{1}{\beta} \log \left( P_n(\mathbf{s})+\epsilon \right) %\left( \frac{P_n(\mathbf{s})}{Z_n}+\epsilon \right)
\end{equation}
where $\beta$ is the inverse temperature, $\gamma$ is the bias factor that broadens the target distribution as in well-tempered Metadynamics \cite{Barducci2008} and $\epsilon$ is a regularization term. %, $\epsilon$ is a regularization term, and $Z_n$ is a normalization constant.
The probability estimate is computed on-the-fly using a weighted kernel density estimation:
\begin{equation}
    P_n(\mathbf{s})=\frac{\sum_k ^n w_k G(\mathbf{s},\mathbf{s_k})}{ \sum_k ^n w_k }
\end{equation}
where the weights $w_k=e^{\beta V_{k-1}(\mathbf{s}_k)}$ are  connected to the value of the bias potential. Once converged, the free energy surface (FES) can be computed as: 
\begin{equation}
    F_n(\mathbf{s})=-\frac{1}{\beta}\log P_n (\mathbf{s})
\end{equation}
and simple reweighting gives access to all the static properties of interest. We refer the reader to \cite{Invernizzi2019} for further details.

Before proceeding to the applications, we summarize the method for clarity:
\begin{enumerate}
    \item Run short unbiased MD runs in the metastable states and compute the descriptors
    \item Construct a CV by training a NN with LDA as the objective function
    \item Use the Deep-LDA CV to enhance the sampling and obtain the FES
\end{enumerate}

\section*{Alanine dipeptide}
The first example that we choose is alanine dipeptide (Ala2), a small molecule often used to benchmark sampling methods. Ala2 has two metastable states that are well described using the pair of Ramachandran angles $\phi$ and $\psi$, which forms a nearly ideal set of CVs. For this reason, the majority of enhanced methods is effective when the angles' fluctuations are enhanced. In order to test Deep-LDA in a less than ideal situation, we opted to use as input all the 45 distances between heavy atoms. This choice makes  Ala2 a non-trivial example since the physical variables $\phi$ and $\psi$ cannot be represented with a linear expression of the interatomic distances and the two states are not linearly separable. We run short unbiased trajectories in the two basins and use this data to train a Deep-LDA CV. The model is then imported in the open-source plug-in PLUMED \cite{Tribello2014} with a custom Pytorch interface and used in OPES. Further details are reported in \ref{sec:S-plumed} and \ref{sec:S-ala2}.

Enhancing the fluctuations of the Deep-LDA CV leads to a very diffusive behavior between the two states, which is comparable to the simulations where the pair of Ramachandran angles is biased (see fig. \ref{fig:S-ala-compare}). This means that Deep-LDA manages to reproduce in an implicit way the two dihedrals which represent the slowest degrees of freedom.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.75\columnwidth]{figures/ala2-fes-iso.png}
  \caption{Free energy surface of Ala2 as a function of the Ramachandran angles, together with the isolines of the Deep-LDA CV, computed from a simulation with a uniform target distribution in this space. The red and blue lines correspond to the regions of the two metastable states used for training, and they are spaced by 0.01. The black ones are extrapolated by the network, with a much larger spacing of 0.2. The isolines are solid or dashed depending on whether they are above or below zero.}
  \label{fig:ala2-fes}
\end{figure}

To illustrate this point further, we present in fig. \ref{fig:ala2-fes} the isolines of the Deep-LDA CV on top of the FES, both projected onto $\phi$ and $\psi$.
As there is no direct correspondence between the dihedral angles and the CV $s$, the isolines have been computed from the conditional probability $p(s\ |\ \phi,\psi)$ in the statistical ensemble generated by an OPES calculation with an uniform target distribution in the $(\phi,\psi)$ space.
%\begin{equation}
%    p(s\ |\ \phi,\psi) = \frac{1}{Z} \int {\text{d}\bar{\phi},\text{d}\bar{\psi}\ \delta(\phi-\bar{\psi}(s))\ \delta(\phi-\bar{\phi}(s))\ s } 
%    \label{eq:isolines}
%\end{equation}
%where $s$ is the Deep-LDA CV and $Z$ a normalization constant. 
When the Deep-LDA fluctuations are enhanced by OPES, the system is driven along the direction perpendicular to the isolines of the CV. It is remarkable how this direction is correlated with the path that connects the two basins in the dihedral's space, managing to trace the underlying free energy landscape (see also fig. \ref{fig:S-ala-isolines}).

We note here that, since Ala2 is a very small molecule, we chose to include in the descriptors set only the distances between heavy atoms. In principle, the Deep-LDA method can be applied to any set of descriptors, including but not limited to angles, dihedrals or hydrogen bonds contacts. 
%In principle, for larger and more complex systems another set of descriptors could be picked by including also angles, dihedrals or hydrogen bonds contacts.

%or other kinds of descriptors which could be useful to describe larger biomolecules or even protein dynamics.

%At last, we computed the ranking of the features from the trained model, based on the magnitude of the weights, see fig. \ref{fig:ala2-ranking}. Besides the distances between neighboring atoms, which are fixed and thus irrelevant, we notice that the Deep-LDA network has given more importance to those distances which are highly correlated with the two Ramachandran angles. On the other hand, the distances at the bottom of the ranking present a low correlation with the two angles. Although is not possible to reproduce the dihedral angles with only planar distances, it is remarkable how Deep-LDA managed to reproduce the angles' behaviour through a combination of distances.

\begin{comment}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.65\columnwidth]{figures/ala2-ranking.png}
  \caption{Ranking of the distances used as input of the Deep-LDA network for Ala2. These values have been calculated by summing the weights modulus of the connections between the inputs and the first layer, multiplied by the standard deviation of the inputs in the training set. They are normalized so that the sum is equal to one. The color of each bar shows the corresponding correlation with the two Ramachandran angles, computed summing the root sum of the squares.}
  \label{fig:ala2-ranking}
\end{figure}
\end{comment}


\section*{Aldol reaction}
The second example is the aldol reaction between vinyl alcohol and formaldehyde. This reaction presents several pathways and products \cite{Yang2017}. Here, for simplicity, we focus on the most probable one, that has a  barrier of $\sim 150$ kJ/mol as estimated in static calculations. This represents a challenging test since it is not obvious whether the reaction's concerted mechanism can be captured with information coming exclusively from unbiased simulations of reactants and products. 
Once again, in the spirit of performing the computation in a blind manner, we build the descriptor set out of all the interatomic distances. We rely on the ability of Deep-LDA to combine them in a meaningful and optimal way and to highlight the most relevant ones.
Previous experience \cite{Rizzi2019} has shown that a good input set for chemical reactions can be obtained from the distances $r_{ij}$ using the following contact function:
\begin{equation}
    c_{ij}(r)=\frac{ 1 - \left(\frac{ r }{ \sigma_{ij} }\right)^{n} }{ 1 - \left(\frac{ r }{ \sigma_{ij} }\right)^{m} }
    \label{eq:contacts}
\end{equation}
where $\sigma_{ij}$ are typical bonding lengths between atoms of species $i$ and $j$. Thus, we express the fact that following the formation and breaking of chemical bonds is key to capturing a chemical process. In this way we still maintain a blind generality while injecting a minimal amount of chemical knowledge. As in the case of modeling interatomic potentials with NNs, the use of chemically informed descriptors allows the NN to learn more easily from the data. See \ref{sec:S-aldol} for the computational details.

As before, we train the Deep-LDA network on unbiased simulations of the two states and use this CV in combination with OPES to enhance the process. One representative trajectory is reported in fig. \ref{fig:aldol}a, which illustrates how the system is reversibly driven from reactants (red) to products (blue).

\begin{figure}[b!]
  \centering
  \includegraphics[width=1
  \columnwidth]{figures/aldol-maxifigure.png}
  \caption{Results of the OPES simulation when enhancing the Deep-LDA CV. (a) Evolution of the carbon-carbon distance between vinyl alcohol and formaldehyde as a function of simulation time. The points are colored according to the Deep-LDA CV. (b) Features ranking according to the magnitude of the weights of the first layer. They are normalized such that the sum is equal to one. The first three distances, separated by a gap from the following ones, are colored in orange. (c) The points correspond to the visited configurations in the plane of the C1-C2 and O1-H distances. As in panel (a), the color is the Deep-LDA CV. The gray dashed lines correspond to the isolines of the free energy surface projected onto this space, while the black solid one corresponds to the minimum free energy path. The teal dotted line is the boundary decision of HLDA. We also reported a few snapshots of the representative structures of the two metastable states and the region between them. (d) Free energy surface projected along the minimum free energy path, computed using the nudged elastic band method \cite{JONSSON1998}.}
  \label{fig:aldol}
\end{figure}

We then focus our attention to the interpretability of the model, by analyzing which features are most important in the Deep-LDA CV. The ranking is defined by summing the modulus of the weights between the input and the first layer, multiplied by the standard deviation of the inputs in the training set. Another option is to calculate the derivatives of the output of the NN with respect to each input, averaged over all inputs in the training set. We found that these two ways of estimating the feature relevance produce similar results.
As shown in fig. \ref{fig:aldol}b, there are three relevant descriptors, separated by a large gap from the following ones. These are the C1-C2 contact where the bond is formed together with the O1-H and O2-H contacts that characterize the proton transfer. This result has been obtained without any \textit{a priori} information on the reaction pathway and it is remarkably in agreement with chemical intuition. 

The FES projected on a pair of these chemically relevant variables presents an easily understandable structure (fig. \ref{fig:aldol}c and \ref{fig:S-aldol-fes}). The two basins are clearly separated and the Deep-LDA CV shows different values in the two basins. As in the Ala2 example, the isolines of Deep-LDA resemble quite closely the ones of the FES. This implies that the direction where the system is driven is correlated with the MFEP, thus acting as a committor-like collective variable. Enhancing the fluctuations along this CV accelerates the sampling along the entire path between the metastable states. This features improves on HLDA that always drives the system in the direction perpendicular to the boundary line drawn in fig. \ref{fig:aldol}c (see also fig. \ref{fig:S-aldol-compare}).

The progress of this work is the realization of a CV that accompanies the evolution of the system along the chemical pathway. We believe this approach can be crucially useful in more complex cases where there are several reaction pathways or multiple reactions and the identification of relevant descriptors is not trivial.

%, while the points explored cluster around the minimum free energy path in this space.  

%Also in light of these findings, we project the free energy on top of different pairs of these three distances (fig. \ref{fig:S-aldol-fes}). Here we focus particularly on the projection along the C1-C2 and O1-H distances, in order to relate them with our CV behavior. In fig. \ref{fig:aldol}c, we report the points visited during the simulation colored by the Deep-LDA CV, together with the isolines of the FES and the minimum free energy path (MFEP). 


\section*{Conclusions}
Deep-LDA is able to compress the information from the metastable states into collective variables. Thanks to the LDA objective function, the distribution of the CV is characterized by a high variance between classes and a low variance within the same class. The non-linearity provided by neural networks allows following the fluctuations between the states, effectively drawing a path in the descriptors space. In principle, the Deep-LDA CV can be used in combination with any CV-based enhanced sampling method. We want to remind the reader that our purpose here is not to find the ideal CV, rather to build a variable which is good enough to promote transitions between the metastable states, given only a limited amount of information. This CV could be further refined in order to closely follow the reaction pathway, either by including weighted data from biased simulations or by combining it with methods designed to extract the slowest relaxation modes \cite{McCarty2017c,Tiwary2016,Chen2019,Wehmeyer2018b,Hernandez2018}. 
Another result is that the Deep-LDA features ranking can be used to identify the relevant descriptors in a data-driven way, as well as filtering them. For all these reasons we believe that our method could be of help in studying a large variety of rare events including but not limited to chemical reactions, nucleation events and ligand-binding processes.



